A Characteristic Function for Shapley-Value-Based Attribution of Anomaly Scores

In anomaly detection, the degree of irregularity is often summarized as a real-valued anomaly score. We address the problem of attributing such anomaly scores to input features for interpreting the results of anomaly detection. We particularly investigate the use of the Shapley value for attributing anomaly scores of semi-supervised detection methods. We propose a characteristic function specifically designed for attributing anomaly scores. The idea is to approximate the absence of some features by locally minimizing the anomaly score with regard to the to-be-absent features. We examine the applicability of the proposed characteristic function and other general approaches for interpreting anomaly scores on multiple datasets and multiple anomaly detection methods. The results indicate the potential utility of the attribution methods including the proposed one.

==> notes.tex <==
\appendix
\newpage

\newcommand{\nonSgivenS}{{\nonS \mid S}}

\newcommand{\vecDecomp}[1]{{\begin{bmatrix} {#1}_S \\ {#1}_\nonS \end{bmatrix}}}
\newcommand{\matDecomp}[1]{{\begin{bmatrix} {#1}_{S,S} & {#1}_{S,\nonS} \\ {#1}_{\nonS,S} & {#1}_{\nonS,\nonS} \end{bmatrix}}}

\newcommand{\ehatcase}[1]{\paragraph{\textcolor{magenta}{[CASE: #1]}}}

% -----------------------------------------------------

\section{Conditional expectation of some common anomaly scores}

\begin{equation*}\begin{aligned}
    \hat{e}_\mathrm{CE}(S; \bm{x})
    &=
    \mathbb{E}_{
        \bm{x}_\nonS
        \sim
        p(\bm{x}_\nonS \mid \bm{x}_S)
    } \left[
        e \left( \vecDecomp{\bm{x}} \right)
    \right]
\end{aligned}\end{equation*}

% ==========

\subsection{Gaussian distributions}

Let the learned Gaussian distribution be
\begin{equation*}
    p(\bm{x}) = \mathcal{N} \left( \vecDecomp{\bm{x}} \mid \bm\mu, \ \bm\Sigma \right),
\end{equation*}
where the parameters are reordered according to index sets $S$ and $\nonS$, that is,
\begin{equation*}\begin{aligned}
    \bm\mu &= \vecDecomp{\bm\mu}, \\
    \bm\Sigma &= \matDecomp{\bm\Sigma}.
\end{aligned}\end{equation*}

\ehatcase{gaussian, energy, condexpt}
The energy (i.e., negative log likelihood) is
\begin{equation*}\begin{aligned}
    e \left( \begin{bmatrix} \bm{x}_S \\ \bm{x}_\nonS \end{bmatrix} \right)
    &=
    \frac{d}2 \log(2\pi)
    + \frac12 \log \left\vert \matDecomp{\bm\Sigma} \right\vert
    \\&\qquad
    + \frac12 \trace \left[ \matDecomp{\bm\Sigma}^{-1} \left(
        \begin{bmatrix}
            (\bm{x}_S-\bm\mu_S) (\bm{x}_S-\bm\mu_S)^\tr &
            (\bm{x}_S-\bm\mu_S) (\bm{x}_\nonS-\bm\mu_\nonS)^\tr \\
            (\bm{x}_\nonS-\bm\mu_\nonS) (\bm{x}_S-\bm\mu_S)^\tr &
            (\bm{x}_\nonS-\bm\mu_\nonS) (\bm{x}_\nonS-\bm\mu_\nonS)^\tr
        \end{bmatrix}
    \right) \right].
\end{aligned}\end{equation*}
The conditional distribution is
\begin{equation*}\begin{aligned}
    p(\bm{x}_\nonS \mid \textcolor{red}{\bm{r}}_S)
    &= \mathcal{N}(\bm{x}_\nonS \mid \bm\mu_{\nonSgivenS}, \ \bm\Sigma_{\nonSgivenS}),
    \\
    \bm\mu_{\nonSgivenS}
    &= \bm\mu_\nonS + \bm\Sigma_{\nonS,S} \bm\Sigma_{\nonS,\nonS}^{-1} (\textcolor{red}{\bm{r}}_S - \bm\mu_S),
    \\
    \bm\Sigma_{\nonSgivenS}
    &= \bm\Sigma_{\nonS,\nonS} - \bm\Sigma_{\nonS,S} \bm\Sigma_{S,S}^{-1} \bm\Sigma_{S,\nonS}.
\end{aligned}\end{equation*}
Hence, $\hat{e}$ becomes
\begin{equation}\begin{aligned}
    &\hat{e}(S; \bm{x}) \underbrace{- \frac{d}2 \log(2\pi) - \frac12 \log \left\vert \matDecomp{\bm\Sigma} \right\vert}_{\text{constant term}}
    \\
    &=
    \frac12 \trace \left[ \matDecomp{\bm\Sigma}^{-1} \left(
        \begin{bmatrix}
            (\bm{x}_S-\bm\mu_S) (\bm{x}_S-\bm\mu_S)^\tr &
            (\bm{x}_S-\bm\mu_S) (\bm\mu_{\nonSgivenS}-\bm\mu_\nonS)^\tr \\
            (\bm\mu_{\nonSgivenS}-\bm\mu_\nonS) (\bm{x}_S-\bm\mu_S)^\tr &
            \bm\Sigma_{\nonSgivenS} + (\bm\mu_{\nonSgivenS}-\bm\mu_\nonS) (\bm\mu_{\nonSgivenS}-\bm\mu_\nonS)^\tr
        \end{bmatrix}
    \right) \right]
    \\
    &=
    \frac12 \trace \left[
        \bm\Sigma_{S\mid\nonS}^{-1} (\bm{x}_S-\bm\mu_S) (\bm{x}_S-\bm\mu_S)^\tr
    \right]
    - \trace \left[
        \bm\Sigma_{S\mid\nonS}^{-1} \bm\Sigma_{S,\nonS} \bm\Sigma_{\nonS,\nonS}^{-1}
        (\bm\mu_{\nonSgivenS}-\bm\mu_\nonS) (\bm{x}_S-\bm\mu_S)^\tr
    \right]
    \\&\qquad
    \underbrace{
    +\frac12 \trace \left[
        \bm{I} + \bm\Sigma_{\nonSgivenS}^{-1} (\bm\mu_{\nonSgivenS}-\bm\mu_\nonS) (\bm\mu_{\nonSgivenS}-\bm\mu_\nonS)^\tr
    \right]
    }_{\text{constant term}},
\end{aligned}\end{equation}
where we used the following facts:
\begin{equation*}\begin{aligned}
    \matDecomp{\bm\Sigma}^{-1}
    &= \begin{bmatrix}
        \bm\Sigma_{S\mid\nonS}^{-1} &
        -\bm\Sigma_{S\mid\nonS}^{-1} \bm\Sigma_{S,\nonS} \bm\Sigma_{\nonS,\nonS}^{-1} \\
        -\bm\Sigma_{\nonS,\nonS}^{-1} \bm\Sigma_{\nonS,S} \bm\Sigma_{S\mid\nonS}^{-1} &
        \bm\Sigma_{\nonSgivenS}^{-1}
    \end{bmatrix},
    \\ \quad\text{where}\quad
    \bm\Sigma_{S\mid\nonS} & = \bm\Sigma_{S,S} - \bm\Sigma_{S,\nonS} \bm\Sigma_{\nonS,\nonS}^{-1} \bm\Sigma_{\nonS,S},
    \\
    \bm\Sigma_{S\mid\nonS}^{-1} &= \bm\Sigma_{S,S}^{-1} + \bm\Sigma_{S,S}^{-1} \bm\Sigma_{S,\nonS} \bm\Sigma_{\nonSgivenS}^{-1} \bm\Sigma_{S,\nonS}^\tr \bm\Sigma_{S,S}^{-1},
    \\ \quad\text{and}\quad
    \bm\Sigma_{\nonSgivenS}^{-1} &= \bm\Sigma_{\nonS,\nonS}^{-1} + \bm\Sigma_{\nonS,\nonS}^{-1} \bm\Sigma_{\nonS,S} \bm\Sigma_{S\mid\nonS}^{-1} \bm\Sigma_{\nonS,S}^\tr \bm\Sigma_{\nonS,\nonS}^{-1}.
\end{aligned}\end{equation*}

% ==========

\subsection{PPCAs}

\ehatcase{ppca, energy, condexpt}
This case is basically the same with the corresponding Gaussian case.
The covariance matrix, $\bm\Sigma$, is given by \emph{reordering} $\bm{C}=\sigma^2\bm{I} + \bm{W}\bm{W}^\tr$ using $S$ and $\nonS$.
The mean, $\bm\mu$, is simply the reordered mean parameter of PPCA.

\ehatcase{ppca, recerr, condexpt}
The reconstruction error is
\begin{equation*}\begin{aligned}
    e \left( \vecDecomp{\bm{x}} \right)
    &= \left\Vert \vecDecomp{\bm{x}} - \left( \matDecomp{\bm{B}} \left( \vecDecomp{\bm{x}} - \vecDecomp{\bm\mu} \right) + \vecDecomp{\bm\mu} \right\Vert_2^2 \right)
    \\
    &= \trace \left[
        \left( \bm{I} - \matDecomp{\bm{B}} \right)
        \begin{bmatrix}
            (\bm{x}_S-\bm\mu_S) (\bm{x}_S-\bm\mu_S)^\tr & (\bm{x}_S-\bm\mu_S) (\bm{x}_\nonS-\bm\mu_\nonS)^\tr \\
            (\bm{x}_\nonS-\bm\mu_\nonS) (\bm{x}_S-\bm\mu_S)^\tr & (\bm{x}_\nonS-\bm\mu_\nonS) (\bm{x}_\nonS-\bm\mu_\nonS)^\tr
        \end{bmatrix}
    \right],
\end{aligned}\end{equation*}
where the submatrices of $\bm{B}$ is obtained by reordering $\bm{W} (\bm{W}^\tr \bm{W})^{-1} \bm{W}^\tr$ (or equivalently, computing the similar matrix from a reordered $\bm{W}$).
Hence, $\hat{e}$ becomes
\begin{equation}\begin{aligned}
    \hat{e}(S;\bm{x})
    &=
    \trace \left[
        \left( \bm{I} - \matDecomp{\bm{B}} \right)
        \begin{bmatrix}
            (\bm{x}_S-\bm\mu_S) (\bm{x}_S-\bm\mu_S)^\tr &
            (\bm{x}_S-\bm\mu_S) (\bm\mu_{\nonSgivenS}-\bm\mu_\nonS)^\tr \\
            (\bm\mu_{\nonSgivenS}-\bm\mu_\nonS) (\bm{x}_S-\bm\mu_S)^\tr &
            \bm\Sigma_{\nonSgivenS} + (\bm\mu_{\nonSgivenS}-\bm\mu_\nonS) (\bm\mu_{\nonSgivenS}-\bm\mu_\nonS)^\tr
        \end{bmatrix}
    \right]
    \\
    &=
    \trace \left[ (\bm{I} - \bm{B}_{S,S}) (\bm{x}_S-\bm\mu_S) (\bm{x}_S-\bm\mu_S)^\tr \right]
    -2 \trace \left[ \bm{B}_{S,\nonS} (\bm\mu_{\nonSgivenS}-\bm\mu_\nonS) (\bm{x}_S-\bm\mu_S)^\tr \right]
    \\
    &\qquad
    \underbrace{
    + \trace \left[ (\bm{I} - \bm{B}_{\nonS,\nonS}) \bm\Sigma_{\nonSgivenS} + (\bm{I} - \bm{B}_{\nonS,\nonS}) (\bm\mu_{\nonSgivenS}-\bm\mu_\nonS) (\bm\mu_{\nonSgivenS}-\bm\mu_\nonS)^\tr \right]
    }_{\text{constant term}}
\end{aligned}\end{equation}
Note that $\bm\mu_{\nonSgivenS}$ and $\bm\Sigma_{\nonSgivenS}$ depend on $\bm\mu$ (reordered), $\bm{W}$ (reordered), and $\sigma^2$ of the learned PPCA.

% ==========

\newpage

\subsection{GMMs}

Let the learned mixture of Gaussian distributions be
\begin{equation*}
    p(\bm{x})
    = \sum_{k=1}^K \pi_k \cdot
    \mathcal{N}(\bm{x} \mid \bm\mu_k, \ \bm\Sigma_k).
\end{equation*}
The energy is
\begin{equation*}
    e \left( \vecDecomp{\bm{x}} \right) = -\underset{k}{\operatorname{logsumexp}} \left[ \log p(\bm{x} \mid z=k) + \log p(z=k) \right],
\end{equation*}
whose integration with regard to $\bm{x}$ is intractable.

\ehatcase{gaussianmix, energy, condexpt}

The conditional distribution is
\begin{equation*}\begin{aligned}
    p(\bm{x}_\nonS \mid \textcolor{red}{\bm{r}}_S)
    &= \sum_{i=1}^K \pi_{k, \nonSgivenS} \cdot \mathcal{N}(\bm{x}_\nonS \mid \bm\mu_{k, \nonSgivenS}, \ \bm\Sigma_{k, \nonSgivenS}),
    \\
    \bm\mu_{k, \nonSgivenS}
    &= \bm\mu_{k,\nonS} - \bm\Sigma_{k,\nonS,\nonS} \bm\Sigma_{k,\nonS,S}^{-1} (\textcolor{red}{\bm{r}}_S - \bm\mu_{k,S}),
    \\
    \bm\Sigma_{k, \nonSgivenS}
    &= \bm\Sigma_{k,\nonS,\nonS} - \bm\Sigma_{k,\nonS,S} \bm\Sigma_{k,S,S}^{-1} \bm\Sigma_{k,S,\nonS},
    \\
    \pi_{k, \nonSgivenS}
    &= \frac{
        \pi_k \cdot \mathcal{N}(\textcolor{red}{\bm{r}}_S \mid \bm\mu_{k,S}, \ \bm\Sigma_{k,S,S})
    }{
        \sum_{l=1}^K \pi_l \cdot \mathcal{N}(\textcolor{red}{\bm{r}}_S \mid \bm\mu_{l,S}, \ \bm\Sigma_{l,S,S})
    }.
\end{aligned}\end{equation*}
As integrating the energy is intractable, we resort to a Monte Carlo approximation.
That is, ...

\newpage

% ==========

\subsection{VAEs}

Let us consider the case of Gaussian VAEs.
Let the learned VAE's decoder be
\begin{equation*}
    p_\theta(\bm{x} \mid \bm{z}) = \mathcal{N}(\bm{x} \mid \bm{f}(\bm{z}), \ \bm{U}),
\end{equation*}
where $\theta = \{ \bm{U}\in\mathcal{S}_+^d, \ \text{parameters of}~\bm{f}:\mathbb{R}^p\to\mathbb{R}^d \}$.
Let the encoder network be
\begin{equation*}
    q_\psi(\bm{z} \mid \bm{x}) = \mathcal{N}(\bm{z} \mid \bm{g}(\bm{x}), \bm{V}(\bm{x}))
\end{equation*}
and $\psi = \{\text{parameters of}~\bm{g}:\mathbb{R}^d\to\mathbb{R}^p~\text{and}~\bm{V}:\mathbb{R}^d\to\mathcal{S}_+^p\}$.
The negative ELBO is
\begin{equation*}\begin{aligned}
    e \left( \bm{x} \right)
    &=
    -\mathbb{E}_{q_\psi(\bm{z} \mid \bm{x})} \left[
        \log p_\theta(\bm{x} \mid \bm{z}) + \log p(\bm{z}) - \log q_\psi(\bm{z} \mid \bm{x})
    \right]
    \\
    &\approx
    -\frac1l \sum_{j=1}^l \log p_\theta(\bm{x} \mid \bm{f}(\bm{g}(\bm\epsilon^{(j)}, \bm{x})), \ \bm{V})
    + \operatorname{KL} \left( q_\psi(\bm{z} \mid \bm{x}) \,\Vert\, p(\bm{z}) \right)
    \\
    &=
    \underbrace{\frac{d}2 \log(2\pi) + \frac12 \log \vert \bm{V} \vert}_{\text{constant term}}
    \\ &\qquad
    + \frac1{2l} \sum_{j=1}^l \trace \left[
        \bm{V}^{-1} \big( \bm{x} - \bm{f}(\bm{g}(\bm\epsilon^{(j)}, \bm{x})) \big) \big( \bm{x} - \bm{f}(\bm{g}(\bm\epsilon^{(j)}, \bm{x})) \big)^\tr
    \right]
    \\ &\qquad
    + \operatorname{KL} \left( q_\psi(\bm{z} \mid \bm{x}) \,\Vert\, p(\bm{z}) \right)
\end{aligned}\end{equation*}
where the first non-constant term is the reconstruction error.
\begin{center}\color{red}\fbox{TODO: rewrite above}\end{center}

As for the conditional distribution, a point is that $p_\theta(\bm{x}_\nonS \mid \bm{x}_S)$ is decomposed as:
\begin{equation*}
    p_\theta(\bm{x}_\nonS \mid \bm{x}_S)
    = \int p_\theta(\bm{x}_\nonS \mid \bm{z}, \cancel{\bm{x}_S}) p_\theta(\bm{z} \mid \bm{x}_S) \mathrm{d}\bm{z}.
\end{equation*}
As this is intractable, we have to resort to MCMC or further approximation techniques.

\ehatcase{vae, elbo, condexpt, exact (mcmc)}
We can draw samples from $p_\theta(\bm{z} \mid \bm{x}_S) \propto p_\theta(\bm{x}_S \mid \bm{z}) p(\bm{z})$ using rejection sampling or some MCMC techniques.
Then throw them to $p_\theta(\bm{x}_\nonS \mid \bm{z})$, by which we obtain samples from $p(\bm{x}_\nonS \mid \bm{x}_S)$.
%The difficulty of this option is that it needs to run the sampling procedures for every $S \subset N\backslash\{i\}$.
Now let $\tilde{\bm{x}}_{\nonSgivenS}$ be the concatenation of 1) $\bm{x}_S$ and 2) a sample from $p(\bm{x}_\nonS \mid \bm{x}_S)$ \emph{in the original order of features (important!)}.
Finally $\hat{e}$ is approximated as
\begin{equation}
    \hat{e}(S; \bm{x}) \approx \frac1{l'} \sum_{j'=1}^{l'} e \left( \tilde{\bm{x}}_{\nonSgivenS}^{(j')} \right).
\end{equation}

% ↓ 無意味
% \ehatcase{vae, elbo, condexpt, gaussapprox}
% Another option is to approximate the conditional using posterior predictive distribution approximated via the Taylor approximation of $\bm{f}$ around $\bm{z}=\bm{z}^*$, where $\bm{z}^*$ is typically the mode of the posterior.
% That is,
% \begin{equation*}
%     \bm{f}(\bm{z}) \approx \bm{f}(\bm{\bm{z}^*}) + \bm{J}_{\bm{f}}(\bm{z}-\bm{z}^*),
% \end{equation*}
% where $\bm{J}_{\bm{f}}\in\mathbb{R}^{d \times p}$ is the Jacobian matrix of $\bm{f}(\bm{z})$ with regard to $\bm{z}$ at $\bm{z}=\bm{z}^*$.
% Then,
% \begin{equation*}
%     p_\theta(\bm{x} \mid \bm{z})
%     \approx
%     \mathcal{N}(\bm{x} \mid \bm{J}_{\bm{f}}\bm{z} + \bm{f}(\bm{z}^*) - \bm{J}_{\bm{f}}\bm{z}^*, \ \bm{U}),
% \end{equation*}
% Consequently, an approximation of the posterior predictive distribution is
% \begin{multline*}
%     \int p_\theta(\bm{x} \mid \bm{z}) q_\psi(\bm{z} \mid \bm{x}^*) \mathrm{d}\bm{z}
%     \\
%     \approx
%     \int
%         \mathcal{N}(\bm{x} \mid \bm{J}_{\bm{f}}\bm{z} + \bm{f}(\bm{z}^*) - \bm{J}_{\bm{f}}\bm{z}^*, \ \bm{U})
%         \mathcal{N}(\bm{z} \mid \bm{g}(\bm{x}^*), \bm{V}(\bm{x}^*))
%     \mathrm{d}\bm{z}
%     \\
%     = \mathcal{N} ( \bm{x} \mid \bm{J}_{\bm{f}} \bm{g}(\bm{x}^*) + \bm{f}(\bm{z}^*) - \bm{J}_{\bm{f}}\bm{z}^*, \ \bm{U} + \bm{J}_{\bm{f}} \bm{V}(\bm{x}^*) \bm{J}_{\bm{f}} )
%     \quad := p^*(\bm{x}).
% \end{multline*}
% Using this $p^*(\bm{x})$, the remaining issue is to compute an approximation of the negative ELBO $e(\bm{x})$, which is highly nonlinear with regard to $\bm{x}$.
% Here note that the Gauss--Hermite quadrature only works for $d\approx1,2,3$ (and something like that) because the number of grid points increases by $L^d$.
% Therefore, we now resort to a simple Monte Carlo approximation.

% -----------------------------------------------------

\newpage
\section{Getting reasonable baseline}

\subsection{General}

VAEs, GMMs, etc.
\begin{equation*}
    \underset{\Delta}{\text{minimize}} ~ \Vert\Delta\Vert_2^2 + I_{e(\bm{x}+\Delta)=\ebaseline}(\Delta)
\end{equation*}

\subsection{Gaussian distributions}

If $\bm{x} \sim \mathcal{N}(\bm\mu, \bm\Sigma)$, then $\bm{y}:=\bm\Lambda^{-\frac12} \bm{W}^\tr (\bm{x}-\bm\mu) \sim \mathcal{N}(\bm{0},\bm{I})$, where $\bm{W}$ and $\bm\Lambda$ are the eigs of $\bm\Sigma$.
So, first compute
\begin{equation*}
    \bm{y}_\mathrm{bl} = \sqrt{\frac{\ebaseline}{e(\bm{x}^*)}} \bm{y}^*
\end{equation*}
and then compute $\bm{x}_\mathrm{bl} = \bm{W} \bm\Lambda^{\frac12} \bm{y} + \bm\mu$.

\subsection{PPCAs}

\subsubsection{Energy}

Exactly the same with the Gaussian case with $\bm\Sigma=\sigma^2\bm{I}+\bm{W}\bm{W}^\tr$.

\subsubsection{Reconstruction error}

Just interpolate between $\bm{x}^*$ and $\tilde{\bm{x}}$, where $\tilde{\bm{x}}$ is the reconstruction of $\bm{x}^*$, by the ratio of
\begin{equation*}
    r = \sqrt{\frac{\ebaseline}{e(\bm{x}^*)}}.
\end{equation*}
That is, the resulting baseline is $\bm{x}_\mathrm{bl} = \tilde{\bm{x}} + r(\bm{x}^*-\tilde{\bm{x}})$.

\subsection{GMMs (approximation)}

For GMMs, we need the general procedure in principle.
But, as an approximation, we can compute a baseline by first selecting a component that $\bm{x}$ belongs and then compute a baseline using the Gaussian case.


% -----------------------------------------------------

\newpage
\section{Desideratum on characteristic function}

Let the characteristic function be
\begin{equation*}
    v(S; \bm{x}) = \max (\hat{e}(S; \bm{x}), \ e_\mathrm{th}),
\end{equation*}
where $\hat{e}$ is either $\hat{e}_\mathrm{B}$ or $\hat{e}_\mathrm{CE}$.
To ensure the speed-up of the Shapley value computation, we want
\begin{equation*}
    \forall S, \bm{x}, i, e_\mathrm{th},
    \quad
    \hat{e}(S; \bm{x}) \geq e_\mathrm{th}
    \ \Rightarrow \
    \hat{e}(S\cup\{i\}; \bm{x}) \geq e_\mathrm{th}.
\end{equation*}
In other words, we want
\begin{equation*}
    \forall S, \bm{x}, i, e_\mathrm{th},
    \quad
    \hat{e}(S; \bm{x}) \ \text{is non-decreasing wrt.} \ \vert S \vert \ \textcolor{blue}{\text{in} \ \hat{e}(S; \bm{x}) \geq e_\mathrm{th}}.
\end{equation*}
What kind of assumptions on $e$ is needed to ensure the above desideratum on $\hat{e}_\mathrm{B}$ or $\hat{e}_\mathrm{CE}$, for each case?

\medskip\noindent\fbox{\color{red} FOR THE TIME BEING, LET THE DESIDERATUM ITSELF AN ASSUMPTION.}

\subsection{Baseline Shapley (BS)}

\begin{equation*}
    \hat{e}_\mathrm{B}(S\cup\{i\}; \bm{x})
    =
    \overbrace{
    e \left(
        \begin{bmatrix} \bm{x}_S \\ x_i \\ \bm{x}^\mathrm{b}_{\nonS\backslash\{i\}}(\bm{x}) \end{bmatrix}
    \right)
    }^\alpha
\end{equation*}
\begin{equation*}
    \hat{e}_\mathrm{B}(S; \bm{x})
    =
    \overbrace{
    e \left(
        \begin{bmatrix} \bm{x}_S \\ x^\mathrm{b}_i(\bm{x}) \\ \bm{x}^\mathrm{b}_{\nonS\backslash\{i\}}(\bm{x}) \end{bmatrix}
    \right)
    }^\beta
\end{equation*}

\begin{equation*}
    \hat{e}_\mathrm{B}(S\cup\{i\}; \bm{x}) - \hat{e}_\mathrm{B}(S; \bm{x}) = ...
\end{equation*}

...?

\subsection{Conditional Expectation Shapley (CES)}

\begin{equation*}
    \hat{e}_\mathrm{CE}(S\cup\{i\}; \bm{x})
    =
    \mathbb{E}_{
        \bm{x}_{\nonS\backslash\{i\}}
        \sim
        p(\bm{x}_{\nonS\backslash\{i\}} \mid \bm{x}_{S\cup\{i\}})
    } \left[ e \left(
        \begin{bmatrix} \bm{x}_S \\ x_i \\  \bm{x}_{\nonS\backslash\{i\}} \end{bmatrix}
    \right) \right]
\end{equation*}
\begin{equation*}\begin{aligned}
    \hat{e}_\mathrm{CE}(S; \bm{x})
    &=
    \mathbb{E}_{
        \bm{x}_\nonS
        \sim
        p(\bm{x}_\nonS \mid \bm{x}_S)
    } \left[ e \left(
        \begin{bmatrix} \bm{x}_S \\ y_i \\ \bm{x}_{\nonS\backslash\{i\}} \end{bmatrix}
    \right) \right]
    \\
    &=
    \mathbb{E}_{
        \bm{x}_{\nonS\backslash\{i\}}, y_i
        \sim
        p(\bm{x}_{\nonS\backslash\{i\}} \mid \bm{x}_{S\cup\{i\}}) p(x_i \mid \bm{x}_S)
    } \left[ e \left(
        \begin{bmatrix} \bm{x}_S \\ y_i \\ \bm{x}_{\nonS\backslash\{i\}} \end{bmatrix}
    \right) \right]
    \\
    &=
    \mathbb{E}_{y_i \sim p(x_i \mid \bm{x}_S)}
    \left[
        \mathbb{E}_{
            \bm{x}_{\nonS\backslash\{i\}}
            \sim
            p(\bm{x}_{\nonS\backslash\{i\}} \mid \bm{x}_{S\cup\{i\}})
        }
        \left[ e \left(
            \begin{bmatrix} \bm{x}_S \\ y_i \\ \bm{x}_{\nonS\backslash\{i\}} \end{bmatrix}
        \right) \right]
    \right]
\end{aligned}\end{equation*}

...?



==> results/realanom_hitsat3.tex <==

\begin{tabular}{ccC{12mm}C{12mm}C{12mm}C{12mm}C{12mm}C{12mm}C{12mm}C{12mm}}
\toprule
\multicolumn{2}{c}{Setting} & \multicolumn{8}{c}{Hits@3} \\
\cmidrule(lr){1-2}\cmidrule(lr){3-10}
Dataset & Detector & \textsc{marg} & \textsc{SFE} & \textsc{ACE} & \textsc{IG} & \textsc{KSH} & \textsc{wKSH} & \textsc{comp} & \textsc{ASH} 
\\
\midrule
\multirow{4}{*}{\texttt{Thyroid}}
 & \textsl{GMM} & {0.80} & {0.67} & {0.80} & {0.80} & {0.80} & {0.87} & {0.67} & {0.93} \\
 & \textsl{VAE-r} & {1.00} & {1.00} & {1.00} & {1.00} & {0.87} & {0.80} & {1.00} & {1.00} \\
 & \textsl{VAE-e} & --- & --- & {0.93} & {1.00} & {0.87} & {0.80} & {0.67} & {1.00} \\
 & \textsl{DAGMM} & --- & --- & {0.47} & {0.00} & {0.67} & {0.47} & {0.87} & {0.87} \\
\midrule
\multirow{4}{*}{\texttt{U2R}}
 & \textsl{GMM} & {0.89} & {0.82} & {0.44} & {0.89} & {0.62} & {0.61} & {0.85} & {0.89} \\
 & \textsl{VAE-r} & {0.89} & {0.89} & {0.86} & {0.81} & {0.79} & {0.57} & {0.89} & {0.90} \\
 & \textsl{VAE-e} & --- & --- & {0.92} & {0.87} & {0.79} & {0.55} & {0.07} & {0.83} \\
 & \textsl{DAGMM} & --- & --- & {0.60} & {0.02} & {0.55} & {0.61} & {0.81} & {0.56} \\
\midrule
\multirow{4}{*}{\texttt{Musk}}
 & \textsl{GMM} & {0.00} & {0.00} & {0.29} & {0.00} & {0.05} & {0.14} & {0.76} & {0.05} \\
 & \textsl{VAE-r} & {0.05} & {0.05} & {0.29} & {0.10} & {0.19} & {0.14} & {0.76} & {0.10} \\
 & \textsl{VAE-e} & --- & --- & {0.19} & {0.10} & {0.19} & {0.14} & {0.76} & {0.00} \\
 & \textsl{DAGMM} & --- & --- & {0.33} & {0.00} & {0.00} & {0.24} & {0.76} & {0.19} \\
\midrule
\multicolumn{2}{c}{25th percentile} & ({0.24}) & ({0.21}) & {0.32} & {0.01} & {0.19} & {0.21} & {0.74} & {0.17} \\
\multicolumn{2}{c}{50th percentile} & ({0.84}) & ({0.74}) & {0.53} & {0.45} & {0.65} & {0.56} & {0.76} & {0.85} \\
\multicolumn{2}{c}{75th percentile} & ({0.89}) & ({0.87}) & {0.88} & {0.88} & {0.79} & {0.66} & {0.85} & {0.91} \\
\bottomrule
\end{tabular}



==> results/synthanom_auc_na1.tex <==

    \begin{tabular}{ccC{12mm}C{12mm}C{12mm}C{12mm}C{12mm}C{12mm}C{12mm}C{12mm}}
    \toprule
    \multicolumn{2}{c}{Setting} & \multicolumn{8}{c}{AUC} \\
    \cmidrule(lr){1-2}\cmidrule(lr){3-10}
    Dataset & Detector & \textsc{marg} & \textsc{SFE} & \textsc{ACE} & \textsc{IG} & \textsc{KSH} & \textsc{wKSH} & \textsc{comp} & \textsc{ASH} 
    \\
    \midrule
    \multirow{4}{*}{\texttt{Thyroid}}
 & \textsl{GMM} & {0.70} & {0.74} & {0.82} & {0.81} & {0.60} & {0.82} & {0.47} & {0.85} \\
 & \textsl{VAE-r} & {0.83} & {0.83} & {0.85} & {0.83} & {0.69} & {0.82} & {0.83} & {0.83} \\
 & \textsl{VAE-e} & --- & --- & {0.82} & {0.83} & {0.66} & {0.83} & {0.44} & {0.83} \\
 & \textsl{DAGMM} & --- & --- & {0.38} & {0.18} & {0.47} & {0.49} & {0.75} & {0.54} \\
\midrule
\multirow{4}{*}{\texttt{Breastw}}
 & \textsl{GMM} & {0.89} & {0.91} & {0.88} & {0.89} & {0.60} & {0.85} & {0.48} & {0.89} \\
 & \textsl{VAE-r} & {0.82} & {0.82} & {0.79} & {0.92} & {0.78} & {0.88} & {0.89} & {0.87} \\
 & \textsl{VAE-e} & --- & --- & {0.82} & {0.93} & {0.79} & {0.87} & {0.53} & {0.93} \\
 & \textsl{DAGMM} & --- & --- & {0.41} & {0.10} & {0.56} & {0.71} & {0.52} & {0.72} \\
\midrule
\multirow{4}{*}{\texttt{U2R}}
 & \textsl{GMM} & {0.95} & {0.93} & {0.79} & {0.95} & {0.60} & {0.91} & {0.59} & {0.95} \\
 & \textsl{VAE-r} & {0.95} & {0.95} & {0.94} & {0.94} & {0.60} & {0.91} & {0.95} & {0.95} \\
 & \textsl{VAE-e} & --- & --- & {0.93} & {0.95} & {0.61} & {0.91} & {0.41} & {0.94} \\
 & \textsl{DAGMM} & --- & --- & {0.63} & {0.06} & {0.49} & {0.74} & {0.89} & {0.82} \\
\midrule
\multirow{4}{*}{\texttt{Lympho}}
 & \textsl{GMM} & {0.89} & {0.95} & {0.72} & {1.00} & {0.50} & {0.50} & {0.66} & {0.99} \\
 & \textsl{VAE-r} & {0.99} & {0.99} & {0.72} & {0.93} & {0.50} & {0.50} & {0.28} & {0.99} \\
 & \textsl{VAE-e} & --- & --- & {0.72} & {0.95} & {0.50} & {0.50} & {0.28} & {0.93} \\
 & \textsl{DAGMM} & --- & --- & {0.44} & {0.33} & {0.50} & {0.50} & {0.72} & {0.91} \\
\midrule
\multirow{4}{*}{\texttt{Musk}}
 & \textsl{GMM} & {0.72} & {0.70} & {0.69} & {0.82} & {0.70} & {0.98} & {0.50} & {0.99} \\
 & \textsl{VAE-r} & {0.99} & {0.99} & {0.89} & {0.90} & {0.85} & {0.99} & {0.72} & {1.00} \\
 & \textsl{VAE-e} & --- & --- & {0.89} & {0.90} & {0.85} & {1.00} & {0.50} & {0.99} \\
 & \textsl{DAGMM} & --- & --- & {0.60} & {0.28} & {0.56} & {0.72} & {0.50} & {0.70} \\
\midrule
\multirow{4}{*}{\texttt{Arrhythmia}}
 & \textsl{GMM} & {0.91} & {0.86} & {0.88} & {0.92} & {0.72} & {0.93} & {0.43} & {0.89} \\
 & \textsl{VAE-r} & {0.97} & {0.97} & {0.89} & {0.95} & {0.90} & {0.95} & {0.85} & {0.97} \\
 & \textsl{VAE-e} & --- & --- & {0.90} & {0.95} & {0.90} & {0.95} & {0.52} & {0.97} \\
 & \textsl{DAGMM} & --- & --- & {0.50} & {0.11} & {0.64} & {0.66} & {0.48} & {0.71} \\
\midrule
\multicolumn{2}{c}{25th percentile} & ({0.83}) & ({0.83}) & {0.67} & {0.69} & {0.55} & {0.70} & {0.48} & {0.83} \\
\multicolumn{2}{c}{50th percentile} & ({0.90}) & ({0.92}) & {0.80} & {0.90} & {0.60} & {0.84} & {0.52} & {0.92} \\
\multicolumn{2}{c}{75th percentile} & ({0.95}) & ({0.95}) & {0.88} & {0.94} & {0.73} & {0.92} & {0.73} & {0.97} \\
\bottomrule
    \end{tabular}
    


==> results/synthanom_gamma_hitsat1.tex <==

    \begin{tabular}{ccC{13mm}C{13mm}C{13mm}C{13mm}C{13mm}}
    \toprule
    \multirow{2}{*}{Dataset} & \multicolumn{5}{c}{Hits@1} \\
    \cmidrule(lr){2-6}
    & $\gamma=0.001$ & $\gamma=0.01$ & $\gamma=0.1$ & $\gamma=1.0$ & $\gamma=10.0$ 
    \\
    \midrule
    \texttt{Thyroid}  & {0.65} & {0.65} & {0.65} & {0.60} & {0.59} \\
\texttt{Breastw}  & {0.66} & {0.66} & {0.66} & {0.66} & {0.67} \\
\texttt{U2R}  & {0.76} & {0.77} & {0.76} & {0.75} & {0.76} \\
\texttt{Lympho}  & {0.49} & {0.49} & {0.49} & {0.50} & {0.52} \\
\texttt{Musk}  & {0.97} & {0.96} & {0.93} & {0.92} & {0.91} \\
\texttt{Arrhythmia}  & {0.41} & {0.41} & {0.41} & {0.42} & {0.42} \\
\bottomrule
    \end{tabular}
    


==> results/synthanom_gamma_hitsat3.tex <==

    \begin{tabular}{ccC{13mm}C{13mm}C{13mm}C{13mm}C{13mm}}
    \toprule
    \multirow{2}{*}{Dataset} & \multicolumn{5}{c}{Hits@3} \\
    \cmidrule(lr){2-6}
    & $\gamma=0.001$ & $\gamma=0.01$ & $\gamma=0.1$ & $\gamma=1.0$ & $\gamma=10.0$ 
    \\
    \midrule
    \texttt{Thyroid}  & {0.89} & {0.88} & {0.89} & {0.89} & {0.88} \\
\texttt{Breastw}  & {0.88} & {0.88} & {0.87} & {0.85} & {0.86} \\
\texttt{U2R}  & {0.97} & {0.97} & {0.97} & {0.97} & {0.97} \\
\texttt{Lympho}  & {0.98} & {0.98} & {0.98} & {0.97} & {0.99} \\
\texttt{Musk}  & {0.98} & {0.97} & {0.97} & {0.93} & {0.93} \\
\texttt{Arrhythmia}  & {0.52} & {0.53} & {0.53} & {0.53} & {0.53} \\
\bottomrule
    \end{tabular}
    


==> results/synthanom_hitsat1.tex <==

    \begin{tabular}{ccC{12mm}C{12mm}C{12mm}C{12mm}C{12mm}C{12mm}C{12mm}C{12mm}}
    \toprule
    \multicolumn{2}{c}{Setting} & \multicolumn{8}{c}{Hits@1} \\
    \cmidrule(lr){1-2}\cmidrule(lr){3-10}
    Dataset & Detector & \textsc{marg} & \textsc{SFE} & \textsc{ACE} & \textsc{IG} & \textsc{KSH} & \textsc{wKSH} & \textsc{comp} & \textsc{ASH} 
    \\
    \midrule
    \multirow{4}{*}{\texttt{Thyroid}}
 & \textsl{GMM} & {0.35} & {0.31} & {0.57} & {0.50} & {0.25} & {0.53} & {0.32} & {0.65} \\
 & \textsl{VAE-r} & {0.61} & {0.61} & {0.62} & {0.61} & {0.37} & {0.65} & {0.61} & {0.61} \\
 & \textsl{VAE-e} & --- & --- & {0.59} & {0.62} & {0.33} & {0.66} & {0.30} & {0.60} \\
 & \textsl{DAGMM} & --- & --- & {0.21} & {0.02} & {0.13} & {0.27} & {0.47} & {0.32} \\
\midrule
\multirow{4}{*}{\texttt{Breastw}}
 & \textsl{GMM} & {0.68} & {0.67} & {0.66} & {0.66} & {0.20} & {0.65} & {0.38} & {0.66} \\
 & \textsl{VAE-r} & {0.51} & {0.51} & {0.61} & {0.73} & {0.53} & {0.72} & {0.63} & {0.68} \\
 & \textsl{VAE-e} & --- & --- & {0.60} & {0.77} & {0.52} & {0.70} & {0.42} & {0.76} \\
 & \textsl{DAGMM} & --- & --- & {0.24} & {0.01} & {0.20} & {0.59} & {0.36} & {0.40} \\
\midrule
\multirow{4}{*}{\texttt{U2R}}
 & \textsl{GMM} & {0.72} & {0.71} & {0.60} & {0.75} & {0.11} & {0.88} & {0.48} & {0.77} \\
 & \textsl{VAE-r} & {0.72} & {0.72} & {0.80} & {0.77} & {0.13} & {0.90} & {0.68} & {0.82} \\
 & \textsl{VAE-e} & --- & --- & {0.71} & {0.82} & {0.13} & {0.88} & {0.29} & {0.80} \\
 & \textsl{DAGMM} & --- & --- & {0.48} & {0.00} & {0.09} & {0.69} & {0.65} & {0.57} \\
\midrule
\multirow{4}{*}{\texttt{Lympho}}
 & \textsl{GMM} & {0.39} & {0.39} & {0.05} & {0.80} & {0.02} & {0.02} & {0.05} & {0.49} \\
 & \textsl{VAE-r} & {0.88} & {0.88} & {0.05} & {0.53} & {0.02} & {0.02} & {0.00} & {0.80} \\
 & \textsl{VAE-e} & --- & --- & {0.05} & {0.54} & {0.02} & {0.02} & {0.00} & {0.80} \\
 & \textsl{DAGMM} & --- & --- & {0.01} & {0.07} & {0.02} & {0.02} & {0.05} & {0.17} \\
\midrule
\multirow{4}{*}{\texttt{Musk}}
 & \textsl{GMM} & {0.03} & {0.03} & {0.17} & {0.20} & {0.10} & {0.90} & {0.05} & {0.96} \\
 & \textsl{VAE-r} & {0.97} & {0.97} & {0.52} & {0.76} & {0.45} & {0.97} & {0.08} & {0.97} \\
 & \textsl{VAE-e} & --- & --- & {0.53} & {0.76} & {0.45} & {0.97} & {0.05} & {0.97} \\
 & \textsl{DAGMM} & --- & --- & {0.03} & {0.01} & {0.03} & {0.36} & {0.05} & {0.20} \\
\midrule
\multirow{4}{*}{\texttt{Arrhythmia}}
 & \textsl{GMM} & {0.13} & {0.13} & {0.12} & {0.27} & {0.02} & {0.33} & {0.03} & {0.41} \\
 & \textsl{VAE-r} & {0.64} & {0.64} & {0.19} & {0.34} & {0.21} & {0.42} & {0.07} & {0.61} \\
 & \textsl{VAE-e} & --- & --- & {0.19} & {0.34} & {0.21} & {0.42} & {0.08} & {0.62} \\
 & \textsl{DAGMM} & --- & --- & {0.07} & {0.00} & {0.00} & {0.12} & {0.03} & {0.10} \\
\midrule
\multicolumn{2}{c}{25th percentile} & ({0.38}) & ({0.37}) & {0.11} & {0.17} & {0.03} & {0.32} & {0.05} & {0.47} \\
\multicolumn{2}{c}{50th percentile} & ({0.62}) & ({0.62}) & {0.36} & {0.54} & {0.13} & {0.62} & {0.18} & {0.64} \\
\multicolumn{2}{c}{75th percentile} & ({0.72}) & ({0.71}) & {0.60} & {0.75} & {0.27} & {0.76} & {0.43} & {0.80} \\
\bottomrule
    \end{tabular}
    

